Learning Output Embeddings in Structured Prediction

A powerful and flexible approach to structured prediction consists in embedding the structured objects to be predicted into a feature space of possibly infinite dimension by means of output kernels, and then, solving a regression problem in this output space. A prediction in the original space is computed by solving a pre-image problem. In such an approach, the embedding, linked to the target loss, is defined prior to the learning phase. In this work, we propose to jointly learn a finite approximation of the output embedding and the regression function into the new feature space. For that purpose, we leverage a priori information on the outputs and also unexploited unsupervised output data, which are both often available in structured prediction problems. We prove that the resulting structured predictor is a consistent estimator, and derive an excess risk bound. Moreover, the novel structured prediction tool enjoys a significantly smaller computational complexity than former output kernel methods. The approach empirically tested on various structured prediction problems reveals to be versatile and able to handle large datasets.

==> Source/3-2-theory_new.tex <==
%\subsection{Theoretical Analysis}

% JR: I don't think this sentence adds any information beyond the previous section
%Predictions are done thanks to the estimations $ h(x) \in \R^p $ through a  projection $\tilde g $ and then a decoding $d$. 
From a statistical viewpoint we 
%recall that the goal is to control 
are interested in controlling the {\em expected risk} of the estimator $f = d \circ \tilde g \circ h$, that for the considered loss corresponds to 
$$
\mathcal{R}(f) = \E_{X,Y}[\|\psi(f(X)) - \psi(Y)\|^2_{\bmHy}].
$$
Interpreting the decoding step in the context of structured prediction, we can leverage the so called {\em comparison inequality} from \cite{Ciliberto2016}. This inequality is applied for our case in the next lemma and relates the excess-risk of $f = d \circ \tilde g \circ h $ to the $L^2$ distance of $\tilde g \circ \hat h$ to $h^*_{\psi}$ (see \cite{Ciliberto2016} for more details on structured prediction and the comparison inequality).
\begin{restatable}{lemma}{cil}
\label{lm:comparison}
For every measurable $\hat h: \bmX \rightarrow \R^p, \tilde g: \R^p \rightarrow \bmHy$, $f = d \circ \tilde g \circ \hat h$, 
\begin{align*}
    \mathcal{R}(f) - \mathcal{R}(f^*) \leq c(\psi) ~ \sqrt{\E_X\|\tilde g \circ \hat h(X) - h^*_{\psi}(X) \|^2_{\bmHy}}
\end{align*}
with $c(\psi) = 2 \sqrt{2Q^2 + Q^4 + 1}$, $Q = \sup_{y \in \bmY} \|\psi(y)\|^2$.
\end{restatable}
It is possible to apply the comparison inequality, since the considered loss function $\Delta(y,y') = \|\psi(y) - \psi(y')\|^2_{\bmHy}$ belongs to the wide family of SELF losses \citep{Ciliberto2016} for which the comparison inequality holds. A loss is SELF if it satisfies the {\em implicit embedding property} \citep{ciliberto2020general}, i.e. there exists an Hilbert space ${\cal V}$ and two feature maps $\gamma, \theta: {\cal Y} \to {\cal V}$ such that
$$\Delta(y,y') = \left\langle\gamma(y),\theta(y')\right\rangle_{\cal V}, \quad \forall ~ y,y' \in {\cal Y}.$$
In our case the construction is direct and corresponds to ${\cal V} = {\bmH_y} \oplus \R \oplus \R$, $\gamma(y) = (\sqrt{2} \psi(y), \|\psi(y)\|_{\bmHy}^2, 1)$ and $\theta(y') = (-\sqrt{2} \psi(y'), 1, \|\psi(y')\|_{\bmHy}^2)$.

Intuitively, the idea of output embedding learning, is to find a new embedding that provides an easier regression task while being still able to predict in the initial regression space. In our formulation this is possible due to introduction of $\tilde g$ and a suitable choice of $\bmG, \tilde \bmG$. In this construction, with the orthogonal decoding $ \tilde g: z \in \R^p \rightarrow \tilde G z \in \bmHy $ described in \ref{subsec:oel_linear}$, \tilde g \circ h $ decomposes into two parts:
\begin{equation}\label{eq:risk-decomposition}
\begin{split}
\underbrace{\E_X[\|\tilde g \circ \hat h_g(X) - h^*_{\psi}(X) \|^2]}_{\text{initial regression problem}} &= \underbrace{\E_X[\|\tilde g \circ \hat h_{g}(X) - \tilde g \circ h^*_{g}(X) \|^2]}_{\text{simplified regression problem}} \\& + \underbrace{\E_X[\|\tilde g \circ  h^*_{g}(X) - h^*_{\psi}(X) \|^2]}_{\text{reconstruction error}}
\end{split}
\end{equation}
In the case of KRR, and arbitrary set of encoding function $\bmG$ from $ \R^p $ to $\bmHy$, the left term expresses as KRR excess-risk on a linear subspace of $\bmH_y$ of dimension $p$ . For the right term, defining the covariance $M_c:\bmHy \to \bmHy$ for all $ c \in [0,1]$, 
% In the case of KRR, linear projections $ \tilde g: z \in \R^p \rightarrow \tilde G z \in \bmHy $, and arbitrary set of function $\bmG$ from $ \R^p $ to $\bmHy$, the left term expresses as KRR excess-risk on a linear subspace of $\bmH_y$ of dimension $p$ . For the right term, defining the covariance $M_c:\bmHy \to \bmHy$ for all $ c \in [0,1]$, 
\[M_{c} = c\E_{x}(h^*(x) \otimes h^*(x)) + (1-c) \E_{y}(\psi(y) \otimes \psi(y))\]
we have the following bound due to Jensen inequality,
\begin{restatable}{lemma}{upb}\label{jensen} Under the assumptions of Lemma~\ref{lm:comparison}, when $\tilde{g}$ is a linear projection, we have
\begin{align*}
    \E_x[\|\tilde g (h^*_{g}(x)) - h^*_{\psi}(x) \|^2] &\leq % c \times \E_{X} [\| G^*G h^*_{\psi}(X) -  h^*_{\psi}(X)\|^2_{\bmHy}] + (1- c) \times \E_Y [\| G^*G\psi(Y) - \psi(Y)\|^2_{\bmH_y}]\\
    %&= 
    \langle I - P,\, M_c \rangle_{\bmH_y \otimes \bmH_y}
\end{align*}
\end{restatable}
The closer $ c $ is to $ 1 $, the tighter is the bound, but having $ c $ close to $ 0 $ could lead to a much easier learning objective. Relying on results on subspace learning in \cite{Rudi2013OnTS} and following their proofs, we bound this upper bound and get the Theorem~\ref{thm:excess-risk}. In particular, we use natural assumption on the spectral properties of the mixed covariance operator $ M_c $ as introduced in \cite{Rudi2013OnTS}. 

\noindent{\bf Assumption 1.}{\em There exist $\omega, \Omega > 0$ and $r > 1$ such that the eigendecomposition of the positive operator $M_c$ has the following form
\begin{align}\label{eq:eig-decay}
M_c = \sum_{j \in \N} \sigma_j u_j \otimes u_j, \quad \omega j^{-r} \leq \sigma_j \leq \Omega j^{-r}.
\end{align}
}
%
The assumption above controls the so called {\em degrees of freedom} of the learning problem. A fast decay of $\sigma_j$ can be interpreted as a problem that is well approximated by just learning the first few eigenvectors (see \cite{caponnetto2007optimal,Rudi2013OnTS} for more details).
%
To conclude, the first part of the r.h.s. of \eqref{eq:risk-decomposition} is further decomposed and then bounded via Lemma~18 of \cite{Ciliberto2016}, leading to Theorem~\ref{thm:excess-risk}. Before we need an assumption on the approximability of $h^*_\psi$. 

\noindent{\bf Assumption 2.} {\em 
The function $h^*_\psi$ satisfies $h^*_\psi \in \bmHy \otimes \bmHx $.
}

The assumption above where $\bmH_x$ is the RKHS associated to $k_x$, guarantees that $h^*_\psi$ is approximable by kernel ridge regression with the given choice of the kernel on the input. The kernel $K(x,x')= Id_{\bmHy} \kerx(x,x')$ satisfies this assumption.
%with the given choice of the kernel on the input.
Now we are ready to state the theorem.
%
% \begin{theorem}[Excess-risk bound, KRR + linear OEL]
% \label{thm:excess-risk}
% Let $ \rho $ be a distribution over $ \bmX \times \bmY $, $ \rho_y $ the marginal of $Y$, $ (x_i, y_i)_{i=1}^n $ be  i.i.d samples from $ \rho $, $ (y_i)_{i=1}^m $ i.i.d samples from $\rho_y$, $ \lambda \leq \kappa^2 := \sup\limits_{x \in \bmX} \|\kerx(x, .)\|_{\bmHx}, \delta > 0$, and $M_{c}$ and $h^*_\psi$ satisfy Assumption 1 and 2. When

% {\color{red} \bf to be updated, when the proof is corrected}
% \begin{equation}
% \label{eq:tradeoff-p}
% p^r \leq  \min\left\{\frac{\omega m}{9 (1-c) Q^2 \log\tfrac{m}{\delta}},\frac{\omega n\lambda^2}{9 c Q^2 \kappa^2 \log(\frac{n}{\delta})},\frac{\omega}{2 c Q\left(1 + \frac{\kappa}{\lambda}\right)\sqrt{\E_x\|\hat h_g(x) - h_\psi^*(x)\|^2} }\right\},
% \end{equation}
% then the following holds with probability at least $1 - \delta$,
% %
% $$\mathcal{R}(\widehat{f}) - \mathcal{R}(f^*) ~~\leq~~  c(\psi) \underbrace{C \frac{Q + R}{\sqrt{\lambda n}}\log^2\tfrac{10}{\delta} + R \sqrt{\lambda}}_{\text{KRR risk on p-dimensional subspace}}  ~~+~~ c(\psi)\underbrace{\sqrt{\frac{\Omega'}{p^{(r-1)/2}}}}_{\text{Reconstruction error}},$$
% where $Q= \sup_{y \in \bmY} \|k(y, .)\|_{\bmH_y}$, $R = \|h^*_\psi\|_{\bmHx \times \bmHy}$,~$C = 4\kappa(1 + (4\kappa^2/\sqrt{\lambda n})^{1/2})$ and $\Omega' = 3\sqrt{3} \Omega^{1/r}(c(1 - 1/r)c(1 + 1/r)c(1/r))^{1/2}$. Note that $C \leq 8\kappa$ when $\lambda \geq 16\kappa^4/n$ .
% \end{theorem}
\begin{restatable}[Excess-risk bound, KRR + OEL]{theorem}{thmer}
\label{thm:excess-risk}
Let $ \rho $ be a distribution over $ \bmX \times \bmY $, $ \rho_y $ the marginal of $Y$, $ (x_i, y_i)_{i=1}^n $ be  i.i.d samples from $ \rho $, $ (y_i)_{i=1}^m $ i.i.d samples from $\rho_y$, $ \lambda \leq \kappa^2 := \sup\limits_{x \in \bmX} \|\kerx(x, .)\|_{\bmHx}, \delta > 0$, and $M_{c}$ and $h^*_\psi$ satisfy Assumption 1 and 2. When
\begin{equation}
\label{eq:tradeoff-p}
p^r \leq  \min\left\{\frac{\omega m}{9 (1-c) \log(m/\delta)},\frac{\omega}{8 c t_n}\right\},
\end{equation}
then the following holds with probability at least $1 - 4\delta$,
%
\begin{equation*}
\begin{split}
    &\sqrt{\E_x(\|\tilde g \circ \hat h_g(x) - h^*_{\psi}(x) \|^2) } \leq \\&\underbrace{C \frac{Q + R}{\sqrt{\lambda n}}\log^2\tfrac{10}{\delta} + R \sqrt{\lambda}}_{\text{KRR on subspace of dim. p}} \qquad + \underbrace{\sqrt{\frac{\Omega'}{p^{r-1}}}}_{\text{Reconstruction error}}
\end{split}
\end{equation*}
where $Q= \sup_{y \in \bmY} \|k(y, .)\|_{\bmHy}$, $R = \|h^*_\psi\|_{\bmHx \times \bmHy}$,~$C = 4\kappa(1 + (4\kappa^2/\sqrt{\lambda n})^{1/2})$,~ $t_n = 5 \max\left(4c^2v_n, 2c v_n, 4cRw_n u_n, 2c w_n^2u_n, 2R^2 u_n\right)$, with $u_n = \frac{4\kappa^2 \log\frac{2}{\delta}}{\sqrt{n}}, v_n = \E_x(\|\hat h_{\psi}(x) - h^*_\psi\|^2)$, $w_n=(\frac{Q}{\lambda \kappa} u_n (1+R) + \lambda R)$. Finally $\Omega' = \Omega q_r$, $q_r$ a constant depending only on $r$ (defined in the proof).
\end{restatable}

The first term in the above bound is the usual bias-variance trade-off that we expect from KRR (c.f. \cite{caponnetto2007optimal}). The second term is an approximation error due to the projection. 

%The resulting bound is constituted by two terms. The first is the usual bias-variance trade-off that we expect from KRR (compare with the result, under the same assumptions of \cite{caponnetto2007optimal}). The second term is an approximation error due to the projection. 
We further see a trade-off in the choice of $c$ when we try to maximize $p$. Choosing $c$ close to one aims to estimate the linear subspace of the $ h^*(x) = \E_{y|x}(\psi(y))$ which is smaller than the one of the $ \psi(y) $ leading to a better eigenvalues decay rate, but the learning is limited by the convergence of the least-square estimator as is clear by the term $v_n$ in Eq.~\eqref{eq:tradeoff-p} (via $ t_n $). Choosing $c$ close to zero leads to completely unsupervised learning of the output embeddings with a smaller eigenvalue decay rate $r$.

Now, in the following corollary, we give a simplified version of the bound (we denote by $a(n) \gtrsim b(n)$ the fact that there exists $C >0$ such that $a(n) \geq C b(n)$ for $n \in \mathbb{N}$).
\begin{restatable}{corollary}{coro}
\label{coro}
Under the same assumptions of Theorem~\ref{thm:excess-risk}, let $\lambda = 1 / \sqrt{n}$. Then, running the proposed algorithm with a number of components 
\[p \gtrsim n^\frac{1}{2r},\] 
is enough to achieve an excess-risk of $\mathcal{R}(\widehat{f}) - \mathcal{R}(f^*)  = O(n^{-(1-\frac{1}{r})/4})$.
\end{restatable}

Note that $n^{-1/4}$ is the typical rate for problems of structured prediction without further assumptions on the problem \cite{Ciliberto2016,ciliberto2020general}. Here it is interesting to note that the more regular the problem is, the more $1 - 1/r \approx 1$, and we can almost achieve $n^{-1/4}$ rate with a a number of components $p \ll n$, in particular $p = n^{1/(2(r-1))}$. Moreover, we expect to find a more subtle trade-off between the KRR error and the approximation error due to projection, since reducing the dimensionality of the output space have a beneficial impact on the degrees of freedom of the problem. We observed this effect from an experimental viewpoint and we expect to observe using a more refined analysis, that we leave as future work.

We want to conclude with a remark on why projecting on $M_c$ with $c \in (0,1)$ should be more beneficial than just projecting on the subspace spanned by the covariance operator associated to $\psi(y)$. Learning the embedding in a supervised fashion is interesting as the principal components of the $ \psi(y) $ may differ from that of the $h_{\psi}^*(x)$. The most basic example: $x \in \R, \psi(y) \in \R^2, x \sim \mathcal{N}(0, \sigma_x^2)$, with the relationship between $ x $ and $\psi(y) = (x,z)$ where $z \sim \mathcal{N}(0, \sigma_z^2)$ independent from $x$ with $\sigma_z^2 > \sigma_x^2$.
In this case unsupervised learning is not able to find the $ 1$-dimensional subspace where the $h^*_{\psi}(x)$ lie, whereas, supervised learning could do so, assuming $ \hat h_{\psi} $ is a good estimation of $h^*_{\psi}$. From this elementary example we could build more complex and realistic ones, by adding any kind of non-isotropic noise $ z $ that change the shape of the $h_{\psi}^*(x)$ subspace. For instance, defining eigenvalue decay of $h_{\psi}^*(x)$ and $ z \in \bmHy $ with $ z $ lower eigenvalue decay, then for $p$ sufficiently large the order of principal components start to change (comparing $h_{\psi}^*(x)$ and $\psi(y) := h_{\psi}^*(x) + z$).
%Analyzing in more detail the contributions of the $p$ we see a trade-off in the choice of $c$ when we try to maximize $p$. Choosing $c$ close to one aims to estimate the linear subspace of the $ h^*(x) = \E_{y|x}(\psi(y))$ which is smaller than the one of the $ \psi(y) $ leading to a better eigenvalues decay rate, but the learning is limited by the convergence of the least-square estimator as clear by the third term of Eq.~\eqref{eq:tradeoff-p}. At the opposite, choosing $c$ close to zero leads to completely unsupervised learning of the output embeddings with a smaller eigenvalue decay rate $r$.

